$\texttt{InfoHier}$: Hierarchical Information Extraction via Encoding and Embedding

Analyzing large-scale datasets, especially involving complex and high-dimensional data like images, is particularly challenging. While self-supervised learning (SSL) has proven effective for learning representations from unlabelled data, it typically focuses on flat, non-hierarchical structures, missing the multi-level relationships present in many real-world datasets. Hierarchical clustering (HC) can uncover these relationships by organizing data into a tree-like structure, but it often relies on rigid similarity metrics that struggle to capture the complexity of diverse data types. To address these we envision $\texttt{InfoHier}$, a framework that combines SSL with HC to jointly learn robust latent representations and hierarchical structures. This approach leverages SSL to provide adaptive representations, enhancing HC's ability to capture complex patterns. Simultaneously, it integrates HC loss to refine SSL training, resulting in representations that are more attuned to the underlying information hierarchy. $\texttt{InfoHier}$ has the potential to improve the expressiveness and performance of both clustering and representation learning, offering significant benefits for data analysis, management, and information retrieval.

==> sections/bg-explicit.tex <==
\vspace{-0.1in}
\subsection{Self-Supervised Learning}
\vspace{-0.1in}

Self-supervised learning (SSL) enables the extraction of meaningful representations from vast, unlabeled data through pretext tasks that encourage models to learn structured data features without explicit labels. Broadly, SSL methods can be categorized as generative, contrastive, or adversarial~\cite{SSL-TKDE, cookbookssl}. Generative SSL methods, such as autoencoders, train an encoder-decoder model to reconstruct inputs by capturing relevant latent features, often using a reconstruction loss to evaluate the similarity between input and output. Techniques like denoising autoencoders~\cite{denoisingAE} or masked autoencoders~\cite{maskedAE} extend this framework by partially corrupting input data and tasking the model with reconstructing the missing information, which enhances robustness. Generative approaches have proven effective in generating or filling in missing data, but can fall short in discriminative tasks.

Contrastive SSL methods, by contrast, focus on relational learning between pairs of inputs, often by maximizing similarity for positive pairs (e.g., augmented views of the same image) and minimizing it for negative pairs (different images). Deep metric methods like CPC \cite{cpc} and SimCLR \cite{simclr} rely on augmentations and similarity objectives to learn useful representations. Other contrastive SSL variants include self-distillation approaches like BYOL \cite{byol}, SimSIAM \cite{simsiam}, and DINO \cite{dino}, which aim to train a model by feeding two different views to two encoders, and mapping one to the other via a predictor. There were also works design the contrastive loss from the idea of canonical correlation analysis (CCA) to infer the relationship between two variables by analyzing their cross-covariance matrices, such as VICReg \cite{vicreg}, Barlow Twins \cite{barlow}, and W-MSE \cite{w-mse}. Researches have also aimed to unify SSL objectives, such as by framing various contrastive losses within a single family of differentiable functions \cite{unifiedCL}, or by theoretically proving SSL from a spectral graph perspective \cite{provablessl, spectralCL}. In parallel, there were also clustering-based SSL methods leveraging unsupervised grouping within the learning process, such as DeepCluster \cite{DeepCluster}, JULE \cite{JULE}, SeLa \cite{SeLa}, and SwAV \cite{swav} which iteratively assign pseudo-labels to data clusters, guiding the network to discover latent structures without explicit labels. However, these methods use flat clustering (such as k-means and nearest neighborhood) assignments as pseudo-labels, neglecting the hierarchy information in input datasets.

% Self-supervised approaches aim at learning from vast unlabeled data, by defining a pretext task based on unlabeled inputs to produce descriptive and intelligible representations. According to their objectives, self-supervised learning can be summarized into three main categories: generative, contrastive, and generative-contrastive (adversarial)~\cite{SSL-TKDE}. These categories can be briefly describe as 
% \begin{itemize}
%     \item Generative: train an encoder to encode input $x$ into latent representation $z$ and a decoder to reconstruct $x$ from $z$.
%     \item Contrastive: train an encoder to encode input $x$ into latent representation $z$ and measure similarity.
%     \item Adversarial: train an encoder-decoder to generate fake samples and a discriminator to distinguish them from real samples.
% \end{itemize}
% Since the adversarial approaches usually have implicit $z$ which is the essential part of our framework, we will focus on the introduction of the other two categories: generative and contrastive. The main difference between these two categories is that the generative methods use a reconstruction loss, the contrastive ones use a contrastive similarity metric. Typical generative methods include autoregressive models such as \cite{auto-reg1, auto-reg2}, whose objective is usually maximizing the likelihood under the forward autoregressive factorization. Another type of generative models are autoencoders (AE) \cite{autoencoders}, whose general goal is to reconstruct (part of) inputs from (corrupted) inputs. The objective of AE is the reconstruction loss that measures how similar are the reconstructions from the original inputs. More recently, there were other variations of AEs such as denoising AE \cite{denoisingAE}, variational AE \cite{varAE}, autoregressive-constrained AE \cite{MADE}, and masked AE \cite{maskedAE}.

% Despite the success of generative SSL in generation tasks, it is recently found far less competitive than contrastive SSL in some classification scenarios because contrastive learning's goal naturally conforms the classification objective. Based on their different ways of defining the contrastive loss, contrastive SSL can be further categorized into four broad families: The Deep Metric Learning Family, The Self-Distillation Family, The Canonical Correlation Analysis Family, and the Masked Image Modeling Family \cite{cookbookssl}. Deep Metric Learning, such as CPC \cite{cpc}, SimCLR \cite{simclr}, is based on the principle of encouraging similarity between positive pairs and dissimilarity between negatives. Self-Distillation methods such as BYOL \cite{byol}, SimSIAM \cite{simsiam}, DINO \cite{dino}, along with their variants rely on another mechanism: feeding two different views to two encoders, and mapping one to the other by means of a predictor. The Canonical Correlation Analysis (CCA) family is named from their usage of CCA, whose goal is to infer the relationship between two variables by analyzing their cross-covariance matrices. This family includes methods like VICReg \cite{vicreg}, Barlow Twins \cite{barlow}, and SwAV \cite{swav}. The Masked Image Modeling tends to mask out portions of an image and teach a model to inpaint them, for instance masked autoencoder \cite{maskedAE} and SimMIM \cite{simmim}.

% While there are several different types of contrastive learning, numerous works have attempted to unify various SSL methods. The generalization ability is proven by an upper bound of classification error rate in \cite{genCSSL}, which also revealed a link between contrastive and covariance-based methods. This direction was further pursued in \cite{duality}, where a covariance-based and contrastive criterion are shown to be equivalent up to normalization. There were also efforts in exploring contrastive self-supervised learning methods from a spectral graph perspective that provide solid theory basis \cite{provablessl, spectralCL}. In \cite{unifiedCL}, it was shown that various contrastive losses can be unified as a general family of loss functions using two monotonously increasing and differentiable scalar functions. Contrastive losses were also investigated from the prospect of maximum entropy principle in \cite{MEC}, which also present a unified view of batch-wise and feature-wise SSL objectives.

% Clustering as a long-existing traditional unsupervised learning methods were also widely explored in SSL. Clustering-based SSL includes DeepCluster \cite{DeepCluster}, JULE \cite{JULE}, LA \cite{LA}, ClusterFit \cite{ClusterFit}, SeLa \cite{SeLa}, SwAV \cite{swav}, SCAN? \cite{}
% However, these methods use flat clustering (such as k-means and nearest neighborhood) assignments as pseudo-labels, neglecting the hierarchy information in input datasets.

\vspace{-0.1in}
\subsection{Clustering}
\vspace{-0.1in}

% Clustering has long been a fundamental task in unsupervised learning, aiming to group data points based on similarity. Traditional methods like K-means and Gaussian Mixture Models (GMMs) perform flat clustering, where data is segmented into non-overlapping groups without capturing any relationships between clusters. While effective for simpler tasks, these methods overlook the hierarchical structure that often exists in real-world datasets, limiting their usefulness for applications that require multi-level grouping.

% Hierarchical Clustering (HC) offers an alternative by organizing data into a tree-like structure, revealing multi-level relationships between clusters. Unlike flat clustering methods, HC doesn't require the number of clusters to be predefined, making it particularly useful for domains where natural hierarchies exist. For instance, in biological taxonomy or document classification, HC can uncover relationships between categories at different levels. However, traditional HC methods rely on fixed distance metrics, which often struggle with complex data, making them sensitive to variations such as image blurring or offsets.

Hierarchical clustering (HC) provides a method for organizing data into nested clusters, capturing multi-level relationships across different groups. Unlike flat clustering methods, HC builds tree-like structures that represent data hierarchies, revealing connections at various levels. Traditional HC approaches rely on predefined distance metrics and linkage-based algorithms, which rigid

Recent works have sought to optimize hierarchical clustering more efficiently, such as through the Dasgupta loss \cite{dasguptaHC}. This loss function measures the quality of a hierarchy by rewarding close intra-cluster points and penalizing distant ones, framing HC as an optimization problem. However, minimizing the Dasgupta loss directly remains challenging, especially in large datasets.
To address these challenges, more recent approaches explore gradient-based hierarchical clustering, which enables the use of gradient descent to optimize hierarchical structures \cite{UFit, gHHC, HypHC}. By using hyperbolic embedding and continuous relaxation cost, these methods allow continuous optimization in the space of discrete binary trees for hierarchical clustering. This opens the opportunity of HC to be integrated with neural networks, facilitating end-to-end learning of both representations and hierarchical relationships.



In this context, combining self-supervised learning (SSL) with HC is a promising direction. SSL, particularly contrastive learning, learns latent representations that can be used to measure similarity more effectively than traditional metrics. The proposed \sname\ framework seeks to jointly train SSL and HC, allowing hierarchical clustering to leverage robust latent representations while enhancing the hierarchical structure learning through SSL, thereby addressing the limitations of fixed metrics in complex datasets.
